Improve Unsupervised Domain Adaptation with Mixup Training

Unsupervised domain adaptation studies the problem of utilizing a relevant source domain with abundant labels to build predictive modeling for an unannotated target domain. Recent work observe that the popular adversarial approach of learning domain-invariant features is insufficient to achieve desirable target domain performance and thus introduce additional training constraints, e.g. cluster assumption. However, these approaches impose the constraints on source and target domains individually, ignoring the important interplay between them. In this work, we propose to enforce training constraints across domains using mixup formulation to directly address the generalization performance for target data. In order to tackle potentially huge domain discrepancy, we further propose a feature-level consistency regularizer to facilitate the inter-domain constraint. When adding intra-domain mixup and domain adversarial learning, our general framework significantly improves state-of-the-art performance on several important tasks from both image classification and human activity recognition.

==> related.tex <==
%The research on domain adaptation can be broadly categorized into supervised domain adaptation (SDA) and unsupervised domain adaptation (UDA) []. Since UDA does not make assumption on the availability of labels on the target domain, it is generally more challenging but also flexible for real-world requirements. In this work, we consider UDA where the target domain is completely unannotated.

%A significant line of UDA research focuses on using deep architectures to learn domain-invariant features to facilitate the transfer. Many early work on this direction emphasize on developing effective discrepancy measures, such as Maximum Mean Discrepancy (MMD) \cite{long2015learning} and Correlation Alingment (CORAL) \cite{sun2016deep}. 
With the advent of adversarial training for generative models (GAN) \cite{goodfellow2014generative}, many research in UDA favors the adoption of a domain discriminator for encouraging domain-invariant representation learning. In order to achieve the maximal confusion of the discriminator for determining the feature origin, the early work of DANN \cite{ganin2016domain} introduces a reverse gradient layer to directly maximize the domain discrimination loss. ADDA framework \cite{tzeng2017adversarial} is proposed to unify several design choices under adversarial learning and a specific architecture is proposed to decouple the encoder of the two domains and adopt the GAN training loss. Moreover, it has been demonstrated that designing better training strategies can enable further adaptation, including separating domain-specific and domain-shared encoders \cite{bousmalis2016domain} and utilizing cycle-consistency constraint \cite{hoffman2018cycada}.
%When applied to medium or high level abstractions of the domain encoder, these measures can induce common feature space shared by both domains through end-to-end learning. 
%in order to quantify the distribution disparity between the two domains. 

Our work follows the recent direction of research which designs specific training constraints to improve target domain performance. This is based on the observation that learning domain-invariant representations alone cannot bridge the performance gap between the two domains \cite{shu2018dirt,chen2019joint}. Intuitively, learning more discriminative features for target domain can lead to improved performance. Since discriminative training is challenging due to the lack of labels in the target domain, \cite{saito2017asymmetric} proposes to utilize predictions from source classifier as pseudo-labels, whereas \cite{chen2019joint} imposes metric-learning style loss for the source domain. The VADA approach \cite{shu2018dirt} incorporates the cluster assumption to steer the decision boundary away from high-density regions in the target domain. Different from these approaches which impose the constraints on the prespecified domain(s) independently, we seek to incorporate both domains in the design of the constraint. By enforcing the constraints across domains, we directly address the target domain performance.
%In \cite{saito2018maximum}, an adversarial approach is taken to identify and avoid generating target features outside the support of source domain data. 

Our proposed approach is built on the recent success of mixup training utilized in semi-supervised learning (SSL) \cite{berthelot2019mixmatch}. Denoting a pair of sample-label tuples as $(x_i,y_i)$, $(x_j, y_j)$, mixup generates augmented tuples as \cite{zhang2017mixup}:
\begin{gather}
    x'=\lambda x_i+(1-\lambda)x_j \nonumber\\
    y'=\lambda y_i+(1-\lambda)y_j \nonumber
\end{gather}
where $\lambda\in[0,1]$. By using the constructed $(x',y')$ for training, mixup encourages linear behavior of the model where linear interpolation in the raw data leads to linear interpolation of predictions. In MixMatch \cite{berthelot2019mixmatch}, mixup plays a central role to jointly exploit the labeled and unlabeled data for SSL. Although the UDA problem considered in this work shares commonality with SSL, the key difference lies on the large discrepancy between the source and target domains. Therefore, different from MixMatch which treats the labeled and unlabeled partitions equally in mixup training, we need to take special care to tackle the domain disparity for the UDA problem.
%as a unique characteristic to
%Although the UDA problem considered in this work shares commonality with SSL, the key difference lies on the large discrepancy between the source and target domains. In this work, we propose strategies to tackle the unique characteristic of UDA in order to faciliate inter-domain mixup training. 
%unique to UDA implies that introducing mixup directly between source and target domains  hinders the efficacy of the linearity assumption

 %Recently, \cite{berthelot2019mixmatch} utilizes mixup as a central role to achieve remarkable performance on semi-supervised learning. In this work, we adopt several components from \cite{berthelot2019mixmatch} as building blocks while making significant modifications to solve the specific challenges in UDA.
%inspired by the simple yet effective \textit{mixup} regularization \cite{zhang2017mixup}. 
